Imitation-based Social Spectrum Sharing

Dynamic spectrum sharing is a promising technology for improving the spectrum utilization. In this paper, we study how secondary users can share the spectrum in a distributed fashion based on social imitations. The imitation-based mechanism leverages the social intelligence of the secondary user crowd and only requires a low computational power for each individual user. We introduce the information sharing graph to model the social information sharing relationship among the secondary users. We propose an imitative spectrum access mechanism on a general information sharing graph such that each secondary user first estimates its expected throughput based on local observations, and then imitates the channel selection of another neighboring user who achieves a higher throughput. We show that the imitative spectrum access mechanism converges to an imitation equilibrium, where no beneficial imitation can be further carried out on the time average. Numerical results show that the imitative spectrum access mechanism can achieve efficient spectrum utilization and meanwhile provide good fairness across secondary users.

==> Convergence1.tex <==
\section{\label{convergence}Convergence of Imitative Spectrum Access On Complete Information Sharing Graph}


\subsection{Dynamics of Imitative Spectrum Access On Complete Information Sharing Graph}
We next study the evolution dynamics of the imitative spectrum mechanism on a complete information sharing graph. This corresponds to the case that all the users are within each other's broadcasting range, and any user can exchange information with any other users. For the ease of exposition, we will focus on the case that the number
of users $N$ is large. Numerical results show that the observations also hold for the case that the number of users is small (see Section \ref{SUP} for details).


In a large user population, it is convenient
to use the population state $\boldsymbol{x}(t)$ to describe the dynamics
of spectrum access. Here $\boldsymbol{x}(t)\triangleq(x_{1}(t),...x_{M}(t))$,
and $x_{m}(t)$ is the fraction of users in the population choosing
channel $m$ to access at decision period $t$.

In the imitative spectrum access mechanism, each user $n$ relies
on its estimated expected throughput $\tilde{U}_{n}(t)$ to
decide whether to imitate other user's channel selection. Due to the
random estimation noise $\omega_{n}$, the evolution of the population
state $\{\boldsymbol{x}(t),\forall t\geq0\}$ is hence stochastic and difficult to
analyze directly. However, when the population of users $N$ is large,
due to the law of large number, such stochastic process can be well
approximated (``averaged out") by its mean-field deterministic trajectory $\{\boldsymbol{X}(t),\forall t\geq0\}$
\cite{key-IM3}. Here $\boldsymbol{X}(t)\triangleq(X_{1}(t),...X_{M}(t))$
is the deterministic population state. Let $P_{i}^{j}(\boldsymbol{X}(t))$
denote the probability that a user choosing channel $i$ in the deterministic
population state $\boldsymbol{X}(t)$ will choose channel $j$ in
next period. According to \cite{key-IM3}, we have
%
\begin{lem}
\label{lem:There-exists-a}There exists a scalar $\delta$, such that
for any bound $\epsilon>0$, decision period $t>0$, and any large enough population size $N$, the maximum difference between the stochastic and deterministic population states over all periods is upper-bounded by $\epsilon$ with an arbitrary large enough probability, i.e., %
\begin{equation}
Pr\{\max_{0\leq\tau\leq t}\max_{m\in\mathcal{M}}|X_{m}(\tau)-x_{m}(\tau)|\leq\epsilon\}\geq 1-e^{-\epsilon^{2}\delta N},\label{eq:DD1}%
\end{equation}
given that $\boldsymbol{X}(0)=\boldsymbol{x}(0)$
and the evolution of the deterministic population state $\{\boldsymbol{X}(t),\forall t\geq0\}$
satisfies%
\begin{equation}
X_{j}(t+1)=\sum_{i=1}^{M}X_{i}(t)P_{i}^{j}(\boldsymbol{X}(t)),\forall j\in\mathcal{M}.\label{eq:DD2}
\end{equation}
\end{lem}

The proof is similar with that in \cite{key-IM3} and hence is omitted
here. As illustrated in Figure \ref{fig:Illustration-of-the}, Lemma
\ref{lem:There-exists-a} indicates that the trajectory of the stochastic
population state $\{\boldsymbol{x}(t),\forall t\geq0\}$ is within a small neighborhood
of the trajectory of the deterministic population state $\{\boldsymbol{X}(t),\forall t\geq0\}$
when the user population $N$ is large enough. Moreover, since the
MLE is unbiased, if the mean-field deterministic dynamics $\{\boldsymbol{X}(t),\forall t\geq0\}$
converge to an equilibrium, the stochastic dynamics $\{\boldsymbol{x}(t),\forall t\geq0\}$
must also converge to the same equilibrium on the time average \cite{key-IM3}.

We now study the evolution dynamics of the deterministic population
state $\{\boldsymbol{X}(t),\forall t\geq0\}$ in (\ref{eq:DD2}). Let $U(m,\boldsymbol{X}(t))=\theta_{m}B_{m}g(NX_{m}(t))$
denote the expected throughput of a user that chooses channel $m$
in the population state $\boldsymbol{X}(t)$. Recall that in the imitative
spectrum access mechanism, each user will randomly choose another
user \rev{to imitate (if that user achieves a higher throughput).}  Thus, we can obtain the probability $P_{i}^{j}(\boldsymbol{X}(t))$
that a user $n$ choosing channel $i$ will imitate another user $n'$
on channel $j$ in the next period as
%
\begin{equation}
P_{i}^{j}(\boldsymbol{X}(t))=X_{j}(t)Pr\{\tilde{U}(j,\boldsymbol{X}(t))>\tilde{U}(i,\boldsymbol{X}(t))\}.\label{eq:DD3}\end{equation}
From (\ref{eq:MLE10}), we have
\begin{multline}
 \tilde{U}(j,\boldsymbol{X}(t))-\tilde{U}(i,\boldsymbol{X}(t)) \\
= U(j,\boldsymbol{X}(t))-U(i,\boldsymbol{X}(t))+\omega_{n'}-\omega_{n},\label{eq:DD4}\end{multline}
where $\omega_{n},\omega_{n'}$ are the random estimation noises with
the probability density function $f(\omega)$. Let $\varpi=\omega_{n}-\omega_{n'}$,
and we can obtain the probability density function of $\varpi$ as\begin{equation}
q(\varpi)=\int_{\underline{\omega}}^{\overline{\omega}}f(\omega)f(\varpi+\omega)d\omega.\label{eq:DD5}\end{equation}
We further denote the cumulative distribution function $\varpi$ as
$Q(\varpi)$, i.e., $Q(\varpi)=\int_{-\infty}^{\varpi}q(s)ds$. Then
from (\ref{eq:DD3}) and (\ref{eq:DD4}), we have for any $j\neq i$,\begin{equation}
P_{i}^{j}(\boldsymbol{X}(t))=X_{j}(t)Q(U(j,\boldsymbol{X}(t))-U(i,\boldsymbol{X}(t))),\label{eq:DD6}\end{equation}
and \begin{equation}
P_{i}^{i}(\boldsymbol{X}(t))=1-\sum_{j\neq i}X_{j}(t)Q(U(j,\boldsymbol{X}(t))-U(i,\boldsymbol{X}(t))).\label{eq:DD7}\end{equation}
Based on (\ref{eq:DD2}), (\ref{eq:DD6}), and (\ref{eq:DD7}), we can
obtain the evolution dynamics of the deterministic population state
$\{\boldsymbol{X}(t)\}$ as
\begin{thm}
For the imitative spectrum access mechanism on a complete information sharing graph, the evolution dynamics of deterministic population
state $\{\boldsymbol{X}(t),\forall t\geq0\}$ are
%
\begin{multline}
\dot{X}_{m}(t) =  X_{m}(t)\sum_{i=1}^{M}X_{i}(t)\left(Q(U(m,\boldsymbol{X}(t))-U(i,\boldsymbol{X}(t))\right. \\
  -\left.Q(U(i,\boldsymbol{X}(t))-U(m,\boldsymbol{X}(t))\right),\label{eq:DD8}\end{multline}
where the derivative is with respect to time $t$.\end{thm}
\begin{proof}
From (\ref{eq:DD2}), (\ref{eq:DD6}), and (\ref{eq:DD7}), we have\begin{eqnarray*}
 &  & \dot{X}_{m}(t) = X_{m}(t+1)-X_{m}(t)\\
% & = & \sum_{i=1}^{M}X_{m}(t)X_{i}(t)P_{i}^{m}(\boldsymbol{X}(t))-X_{m}(t)\\
 & = & \sum_{i\neq m}X_{i}(t)P_{i}^{m}(\boldsymbol{X}(t))-(1-P_{m}^{m}(\boldsymbol{X}(t)))X_{m}(t)\\
 & = & X_{m}(t)\sum_{i\neq m}X_{i}(t)Q(U(m,\boldsymbol{X}(t))-U(i,\boldsymbol{X}(t)))\\
 &  & -X_{m}(t)\sum_{j\neq m}X_{j}(t)Q(U(j,\boldsymbol{X}(t))-U(m,\boldsymbol{X}(t))),\end{eqnarray*}
which completes the proof.
\end{proof}
%
\begin{figure}
\centering
\includegraphics[scale=0.6]{DeteDynamic}
\caption{\label{fig:Illustration-of-the}Illustration of the approximation
of stochastic population state $\boldsymbol{x}(t)$ by deterministic
population state $\boldsymbol{X}(t)$}
\end{figure}


\subsection{\label{convergence}Convergence of Imitative Spectrum Access On Complete Information Sharing Graph}

We now study the convergence of the imitative spectrum access mechanism.
Let $\boldsymbol{x}^{*}\triangleq(x_{1}^{*},...,x_{M}^{*})$ denote
the equilibrium of the imitative spectrum access, and $a_{n}^{*}$
denote the channel chosen by user $n$ in the equilibrium $\boldsymbol{x}^{*}$.
We first introduce the definition of \emph{imitation equilibrium}.
\begin{defn} [\textbf{Imitation Equilibrium}]
\label{def:A-population-state}A population state $\boldsymbol{x}^{*} \rev{=} (x_{1}^{*},...,x_{M}^{*})$
is an imitation equilibrium if and only if for each user $n\in\mathcal{N},$
\begin{equation}
U(a_{n}^{*},\boldsymbol{x}^{*})\geq\max_{a\in\Delta(\boldsymbol{x}^{*})\backslash\{a_{n}^{*}\}}U(a,\boldsymbol{x}^{*}),\label{eq:IM1}\end{equation}
where $\Delta(\boldsymbol{x}^{*})\triangleq\{m\in\mathcal{M}:x_{m}^{*}>0\}$
denotes the set of channels chosen by users in the equilibrium
$\boldsymbol{x}^{*}$.
\end{defn}
\rev{At an imitation equilibrium, no user can further improve its expected throughput by imitating another user.} For the imitative
spectrum access mechanism, we show that
\begin{thm}
\label{thm:For-the-imitative}For the imitative spectrum access mechanism on a complete information sharing graph, the evolution dynamics
of deterministic population state $\{\boldsymbol{X}(t),\forall t\geq0\}$ asymptotically
converge to an imitation equilibrium $\boldsymbol{X}^{*}$ \rev{such that all users achieve the same expected throughput, i.e.,}
\begin{equation}
U(a_{n}^{*},\boldsymbol{X}^{*})=U(a_{n'}^{*},\boldsymbol{X}^{*}),\forall n,n'\in\mathcal{N}.\label{eq:IM2}\end{equation}
\end{thm}

\begin{proof}
To proceed, we first define the following function\begin{equation}
V(\boldsymbol{X}(t))=\sum_{m=1}^{M}\int_{-\infty}^{X_{m}(t)}\theta_{m}B_{m}g(Nz)dz.\label{eq:C1}\end{equation}
We then consider the variation of $V(\boldsymbol{X}(t))$ along the
evolution trajectory of deterministic population state $\{\boldsymbol{X}(t)\}$
in (\ref{eq:DD8}), i.e., differentiating $V(\boldsymbol{X}(t))$
with respective to time $t$,\begin{eqnarray}
 &  & \frac{dV(\boldsymbol{X}(t))}{dt}\nonumber =  \sum_{m=1}^{M}\frac{dV(\boldsymbol{X}(t))}{dX_{m}(t)}\frac{dX_{m}(t)}{dt}\nonumber \\
 & = & \sum_{m=1}^{M}\theta_{m}B_{m}g(NX_{m}(t))\frac{dX_{m}(t)}{dt}\nonumber \\
 & = & \sum_{m=1}^{M}U(m,\boldsymbol{X}(t))X_{m}(t)\sum_{i=1}^{M}X_{i}(t)\nonumber \\
 &  & \times\Big(Q(U(m,\boldsymbol{X}(t))-U(i,\boldsymbol{X}(t))\Big.\nonumber \\
 &  & \Big.-Q(U(i,\boldsymbol{X}(t))-U(m,\boldsymbol{X}(t))\Big)\nonumber \\
 & = & \frac{1}{2}\sum_{m=1}^{M}\sum_{i=1}^{M}X_{m}(t)X_{i}(t)\nonumber \\
 &  & \times\left(U(m,\boldsymbol{X}(t))-U(i,\boldsymbol{X}(t))\right)\nonumber \\
 &  & \times\Big(Q(U(m,\boldsymbol{X}(t))-U(i,\boldsymbol{X}(t))\Big.\nonumber \\
 &  & \Big.-Q(U(i,\boldsymbol{X}(t))-U(m,\boldsymbol{X}(t))\Big).\label{eq:C2}\end{eqnarray}

Since $f(\omega)$ is a probability density function satisfying $f(\omega)>0,\forall\omega\in(\underline{\omega},\overline{\omega})$
and $\int_{\underline{\omega}}^{\overline{\omega}}f(\omega)d\omega=1$,
it follows from (\ref{eq:DD5}) that $q(\varpi)>0,\forall\varpi\in(\underline{\omega}-\overline{\omega},\overline{\omega}-\underline{\omega})$
and $q(\varpi)=0,\forall\varpi\notin(\underline{\omega}-\overline{\omega},\overline{\omega}-\underline{\omega})$.
Hence the cumulated probability function $Q(\varpi)=\int_{-\infty}^{\varpi}q(s)ds$
is strictly increasing for any $\varpi\in(\underline{\omega}-\overline{\omega},\overline{\omega}-\underline{\omega})$,
and further $Q(\varpi)=0,\forall\varpi\in(-\infty,\underline{\omega}-\overline{\omega})$
and $Q(\varpi)=1,\forall\varpi\in(\overline{\omega}-\underline{\omega},+\infty)$. This implies that if $U(m,\boldsymbol{X}(t))\neq U(i,\boldsymbol{X}(t)$,
\begin{eqnarray}
 &  & \left(U(m,\boldsymbol{X}(t))-U(i,\boldsymbol{X}(t))\right)\nonumber \\
 &  & \times\Big(Q(U(m,\boldsymbol{X}(t))-U(i,\boldsymbol{X}(t))\Big.\nonumber \\
 &  & \Big.-Q(U(i,\boldsymbol{X}(t))-U(m,\boldsymbol{X}(t))\Big)>0,\label{eq:C3-1}\end{eqnarray}
and if $U(m,\boldsymbol{X}(t))=U(i,\boldsymbol{X}(t)$, \begin{eqnarray}
 &  & \left(U(m,\boldsymbol{X}(t))-U(i,\boldsymbol{X}(t))\right)\nonumber \\
 &  & \times\Big(Q(U(m,\boldsymbol{X}(t))-U(i,\boldsymbol{X}(t))\Big.\nonumber \\
 &  & \Big.-Q(U(i,\boldsymbol{X}(t))-U(m,\boldsymbol{X}(t))\Big)=0.\label{eq:C4-1}\end{eqnarray}
From (\ref{eq:C2}), (\ref{eq:C3-1}) and (\ref{eq:C4-1}), we have
$\frac{dV(\boldsymbol{X}(t))}{dt}\geq0$. Hence $V(\boldsymbol{X}(t))$
is non-decreasing along the trajectory of the dynamics (\ref{eq:DD8}).
According to \cite{key-IM4}, the evolution dynamics of deterministic
population state $\{\boldsymbol{X}(t), \forall t\geq0\}$ asymptotically converge
to a limit point $\boldsymbol{X}^{*}$ such that $\frac{dV(\boldsymbol{X}^{*})}{dt}=0,$
i.e., \begin{multline}
  X_{m}^{*}X_{i}^{*}\left(U(m,\boldsymbol{X}^{*})-U(i,\boldsymbol{X}^{*})\right)  \\
\times\Big(Q(U(m,\boldsymbol{X}^{*})-U(i,\boldsymbol{X}^{*})-Q(U(i,\boldsymbol{X}^{*})-U(m,\boldsymbol{X}^{*})\Big)=0.\label{eq:C5}\end{multline}
By (\ref{eq:C4-1}), we must have $U(m,\boldsymbol{X}^{*})=U(i,\boldsymbol{X}^{*}),\forall m,i\in\Delta(\boldsymbol{x}^{*}).$
Since $a_{n}^{*},a_{n'}^{*}\in\Delta(\boldsymbol{x}^{*})$, we thus
have $U(a_{n}^{*},\boldsymbol{X}^{*})=U(a_{n'}^{*},\boldsymbol{X}^{*})$.
\end{proof}

According to Lemma \ref{lem:There-exists-a}, we know that the
stochastic imitative spectrum access dynamics $\{\boldsymbol{x}(t),\forall t\geq0\}$
will be \rev{attracted} into a small neighborhood around the imitation
equilibrium $\boldsymbol{X}^{*}$. Moreover, since the imitation equilibrium
$\boldsymbol{X}^{*}$ is also the mean field equilibrium of stochastic
dynamics $\{\boldsymbol{x}(t),\forall t\geq0\}$, the stochastic dynamics $\{\boldsymbol{x}(t),\forall t\geq0\}$
hence converge to the imitation equilibrium $\boldsymbol{X}^{*}$
on the time average, i.e., $\lim_{t\rightarrow\infty}\frac{\sum_{\tau=1}^{t}x_{m}(\tau)}{t}=X_{m}^{*},\forall m\in\mathcal{M}$.

Interestingly, when the set of chosen channels \rev{is the set of all channels, i.e., }$\Delta(\boldsymbol{X}^{*})=\mathcal{M},$
it is easy to verify that the imitation equilibrium $\boldsymbol{X}^{*}$
is a Nash equilibrium, since no user can improve its payoff by changing
its channel unilaterally. Numerical results show that when the number
of users $N$ is large, the imitative spectrum access mechanism
converges to a Nash equilibrium. More precisely, this is because that the
probability that a channel is not chosen by any users equals to $(M-1)^{-N}$,
which decreases exponentially with the number of users $N$. Intuitively, users' behaviors become diverse when the user population is large. Imitation with diversity can drive a balance between exploitation and exploration and hence lead the system to an efficient and stable equilibrium (i.e., Nash equilibrium wherein no user can further improve its throughput by  changing its channel unilaterally). 

==> Figure.tex <==
\clearpage


%\begin{figure}[t]
%\centering
%\includegraphics[scale=0.75]{time_slot}
%\caption{\label{fig:Time-slot-structure} Multiple stages in a single time slot.}
%\end{figure}
%
%\begin{figure}[t]
%\centering
%\includegraphics[scale=0.75]{Time}
%\caption{\label{fig:time}The period structure of maximum likelihood estimation of various system parameters.}
%\end{figure}



%
%\begin{figure}[t]
%\centering
%\includegraphics[scale=0.8]{ClusterG}
%\caption{\label{fig:An-illustration-of}An illustration of cluster-based representation
%of information sharing graph}
%\end{figure}
%
%
%\begin{figure}[t]
%\centering
%\includegraphics[scale=0.8]{DeteDynamic}
%\caption{\label{fig:Illustration-of-the}Illustration of the approximation
%of stochastic population state $\boldsymbol{x}(t)$ by deterministic
%population state $\boldsymbol{X}(t)$}
%\end{figure}



%\begin{figure}[t]
%\centering
%\includegraphics[scale=0.5]{fig1}
%\caption{\label{fig:Evolution-of-stochastic}Evolution of stochastic population
%state with user population $N=1000,800,500$ and $200$}
%\end{figure}
%
%
%\begin{figure}[t]
%\centering
%\includegraphics[scale=0.5]{fig2}
%\caption{\label{fig:Evolution-of-time}Evolution of time average population
%state and user's payoff with user population $N=500$ and $200$}
%\end{figure}

%\begin{figure}[t]
%\centering
%\includegraphics[scale=0.65]{Cluster}
%\caption{\label{fig:Four-different-types}Two types of cluster-based
%graphs with $z_{k}$ representing the number of users in each cluster
%$k$}
%\end{figure}
%
%
%%
%\begin{figure}[t]
%\centering
%\includegraphics[scale=0.5]{f1}
%\caption{\label{fig:Users'-average-throughputs}Users' average throughputs and fractions of users on different channels
%on two types of cluster-based graphs in Figure \ref{fig:Four-different-types}}
%\end{figure}

%
%\begin{figure}[t]
%\centering
%\includegraphics[scale=0.35]{20Graph}
%\caption{\label{fig:Different-information-sharing}Different information sharing
%graphs with the number of users $N=20$. Graphs (a) and (b) are from \cite{watts1998collective}.}
%\end{figure}
%
%\begin{figure}[t]
%\centering
%\includegraphics[scale=0.5]{f2}
%\caption{\label{fig:Users'-average-throughputs2}Imitative spectrum access without innovation
%on different information sharing graphs in Figure \ref{fig:Different-information-sharing} with the number of users $N=20$}
%\end{figure}
%
%\begin{figure}[t]
%\centering
%\includegraphics[scale=0.5]{f3}
%\caption{\label{fig:Users'-average-throughputs3} Imitative spectrum access with innovation
%on different information sharing graphs in Figure \ref{fig:Different-information-sharing} with the number of users $N=20$}
%\end{figure}





%\begin{figure}[t]
%\centering
%\includegraphics[scale=0.45]{150Graph1}
%\caption{\label{fig:A-square-area}A square area of a length of $250$ m with
%$150$ scattered users. Each user has a information transmission range
%$\delta=40$ m. Each user can share information with those users that
%are connected with it by an edge.}
%\end{figure}
%
%
%\begin{figure}[t]
%\centering
%\includegraphics[scale=0.45]{f5}
%\caption{\label{fig:Users'-average-throughputs-1}Users' average throughputs and fractions of users on different channels
%on the information sharing graph in Figure \ref{fig:A-square-area}}
%\end{figure}

